SCORES: Shape Composition with Recursive Substructure Priors

We introduce SCORES, a recursive neural network for shape composition. Our network takes as input sets of parts from two or more source 3D shapes and a rough initial placement of the parts. It outputs an optimized part structure for the composed shape, leading to high-quality geometry construction. A unique feature of our composition network is that it is not merely learning how to connect parts. Our goal is to produce a coherent and plausible 3D shape, despite large incompatibilities among the input parts. The network may significantly alter the geometry and structure of the input parts and synthesize a novel shape structure based on the inputs, while adding or removing parts to minimize a structure plausibility loss. We design SCORES as a recursive autoencoder network. During encoding, the input parts are recursively grouped to generate a root code. During synthesis, the root code is decoded, recursively, to produce a new, coherent part assembly. Assembled shape structures may be novel, with little global resemblance to training exemplars, yet have plausible substructures. SCORES therefore learns a hierarchical substructure shape prior based on per-node losses. It is trained on structured shapes from ShapeNet, and is applied iteratively to reduce the plausibility loss.We showresults of shape composition from multiple sources over different categories of man-made shapes and compare with state-of-the-art alternatives, demonstrating that our network can significantly expand the range of composable shapes for assembly-based modeling.

==> figures/train_adjust.tex <==
\begin{figure}[t!] \centering
	\begin{overpic}[width=1.0\linewidth,tics=10]{train_adjust}%,grid
    %\put(18,5){\small (a)}
    %\put(59,-3){\small (b)}
    %\put(85,-3){\small (c)}
	\end{overpic}
    \caption{Joint training of substructure model (latent space dictionary learning) and geometric adjustment model (denoising network training). Two losses, VQ representation loss and OBB-wise self-reconstruction loss, are minimized. The network connections for bottom-up encoding and top-down decoding are simplified into grey double arrows, for clarity.}
    \label{fig:trainadjust}
    \vspace{-7pt}
\end{figure}


==> figures/train_gen.tex <==
\begin{figure}[t!] \centering
	\begin{overpic}[width=1.0\linewidth,tics=10]{train_gen}%,grid
    %\put(18,5){\small (a)}
    %\put(59,-3){\small (b)}
    %\put(85,-3){\small (c)}
	\end{overpic}
    \caption{Training of synthesis model with the substructure corresponding to the internal node shaded in red. Since this model shares the encoder with the geometric adjustment model, it simply clones and fine-tunes the decoder trained by the latter. The training minimizes OBB-wise self-reconstruction loss.}
    \label{fig:traingen}
    \vspace{-7pt}
\end{figure}

